Quantum Orbital Minimization Method for Excited States Calculation on Quantum Computer

We propose a quantum-classical hybrid variational algorithm, the quantum orbital minimization method (qOMM), for obtaining the ground state and low-lying excited states of a Hermitian operator. Given parameterized ansatz circuits representing eigenstates, qOMM implements quantum circuits to represent the objective function in the orbital minimization method and adopts classical optimizer to minimize the objective function with respect to parameters in ansatz circuits. The objective function has orthogonality implicitly embedded, which allows qOMM to apply a different ansatz circuit to each reference state. We carry out numerical simulations that seek to find excited states of the $\text{H}_{2}$, $\text{LiH}$, and a toy model consisting of 4 hydrogen atoms arranged in a square lattice in the STO-3G basis and UCCSD ansatz circuits. Comparing the numerical results with existing excited states methods, qOMM is less prone to getting stuck in local minima and can achieve convergence with more shallow ansatz circuits.

==> Makefile <==
name=revised_paper

all: $(name).pdf

$(name).pdf: $(name).tex revision.sty
	pdflatex $(name)
	bibtex   $(name).aux
	pdflatex $(name)
	pdflatex $(name)

reply:
	pdflatex ReplyLetter
	pdflatex ReplyLetter

clean:
	rm -f $~ *.aux *.idx *.log *.blg *.bbl *.toc *.dvi *.ps *.out *.gz \
			 *.fdb_latexmk *.fls
cleanless:
	rm -f $~ *.aux *.idx *.log *.blg *.toc *.dvi *.ps *.out *.gz \
			 *.fdb_latexmk *.fls
cleanall:
	rm -f $~ *.aux *.idx *.log *.blg *.bbl *.toc *.dvi *.ps *.out *.gz \
			 *.fdb_latexmk *.fls \
	         figure/*-eps-converted-to.pdf $(name).pdf \
			 ReplyLetter.pdf
zip:
	zip $(name).zip *.sty *.bib *.bbl *.tex *.pdf figures/*.eps \
		figures/*.svg

